Sparse Fuse Dense: Towards High Quality 3D Detection with Depth Completion

Current LiDAR-only 3D detection methods inevitably suffer from the sparsity of point clouds. Many multi-modal methods are proposed to alleviate this issue, while different representations of images and point clouds make it difficult to fuse them, resulting in suboptimal performance. In this paper, we present a novel multi-modal framework SFD (Sparse Fuse Dense), which utilizes pseudo point clouds generated from depth completion to tackle the issues mentioned above. Different from prior works, we propose a new RoI fusion strategy 3D-GAF (3D Grid-wise Attentive Fusion) to make fuller use of information from different types of point clouds. Specifically, 3D-GAF fuses 3D RoI features from the couple of point clouds in a grid-wise attentive way, which is more fine-grained and more precise. In addition, we propose a SynAugment (Synchronized Augmentation) to enable our multi-modal framework to utilize all data augmentation approaches tailored to LiDAR-only methods. Lastly, we customize an effective and efficient feature extractor CPConv (Color Point Convolution) for pseudo point clouds. It can explore 2D image features and 3D geometric features of pseudo point clouds simultaneously. Our method holds the highest entry on the KITTI car 3D object detection leaderboard, demonstrating the effectiveness of our SFD. Codes are available at https://github.com/LittlePey/SFD.

==> figText/visualization.tex <==
\begin{figure*}[t]
	\vspace{-5pt}
	\centering
	\includegraphics[width=1\linewidth]{figures/visualization}
	\caption{Comparison between SFD and Voxel-RCNN. For the visualization of SFD and Voxel-RCNN, we use pseudo clouds and raw clouds, respectively. We show true positives in green and false positives in indigo. The ground-truth boxes and raw LiDAR points inside the boxes are rendered in red. Green arrows represent that our predictions are more accurate, and indigo arrows represent false positives of Voxel-RCNN. The figures beside BEV boxes represent the score and 3d iou.}
	\vspace{-10pt}
	\label{fig:visualization}
\end{figure*}
